Lattice Gauge Theories at the Energy Frontier

This White Paper has been prepared as a planning document for the Division of High Energy Physics of the U. S. Department of Energy. Recent progress in lattice-based studies of physics beyond the standard model is summarized, and major current goals of USQCD research in this area are presented. Challenges and opportunities associated with the recently discovered 126 GeV Higgs-like particle are highlighted. Computational resources needed for reaching important goals are described. The document was finalized on February 11, 2013 with references that are not aimed to be complete, or account for an accurate historical record of the field.

==> authors.tex <==
%\author{Thomas Appelquist, Richard Brower, Simon  Catterall, George Flemming, Anna Hasenfratz, 
%Julius Kuti, Ethan O'Neil, and David Schaich}
